Systematic analysis of requirements for socially acceptable service robots

In modern society, service robots are increasingly recognized for their wide range of practical applications. In large and crowded social spaces, such as museums and hospitals, these robots are required to safely move in the environment while exhibiting user-friendly behavior. Ensuring the safe and socially acceptable operation of robots in such settings presents several challenges. To enhance the social acceptance in the design process of service robots, we present a systematic analysis of requirements, categorized into functional and non-functional. These requirements are further classified into different categories, with a single requirement potentially belonging to multiple categories. Finally, considering the specific case of a receptionist robotic agent, we discuss the requirements it should possess to ensure social acceptance.

==> Tables/categories_requirement.tex <==
\begin{table}[tb]
    \centering
    \begin{tabular}{|p{2.0cm}|p{10.0cm}|}
        \hline
        \cellcolor{cyan!25}Requirement category  & \cellcolor{cyan!25}Explanation  \\
        \hline
        Environment & Includes requirements that address the environment in which the XR system operates, including physical and digital environments\\
        \hline
        Interaction & Includes requirements that address how the user interacts with the XR system, such as text input, touchscreen, voice commands, and gestures\\
        \hline
        Operability &  Includes requirements related to the functionality and stability of hardware and software components, which ensure the smooth operation and reliability of the XR system \\
        \hline
        Perception & Includes requirements for sensory inputs used by the XR system, including computer vision, sensors, and other data sources for interpreting the environment\\
        \hline
        Privacy & Includes requirements for measures to protect sensitive data, including personal and confidential information, ensuring proper handling and compliance with privacy regulations\\
        \hline
        Regulations & Includes requirements regarding adherence to company policies, industry standards and legal requirements governing the use and deployment of XR systems \\
        \hline
        Safety & Includes requirements to ensure that the XR system does not present risks or hazards to users, minimizing the potential for injury or trauma during operation \\
        \hline
    \end{tabular}
    \caption{Categorization of the requirements}
    \label{tab:categories_requirement}
\end{table}


 
 

 

==> requirements.tex <==
\subsection{ENVIRONMENT REQUIREMENTS}
\label{subsec:env_req}
\subsubsection{FR}
\label{subsec:env_FR}
\begin{itemize}
    \item \textbf{Manifest in 3D mode (on any screen)}: the system (e.g.: 3D avatar) should be capable of appearing on screens across various devices such as phones, tablets, and laptop computers, ensuring responsiveness and user interface (UI) adaptability.
   
    \item \textbf{Manifest in 3D mode (in MR/AR)}: the XR system (e.g.: 3D avatar) should be capable of appearing as a accurately positioned MR object on a head-mounted display (HMD) to facilitate spatial perception.
    
    \item \textbf{Follow occlusion standards in MR mode}: the XR system should have the capability to disappear behind a shelf, wall, or obstruct the view of a person or object in MR mode to enhance human interaction and maintain a realistic environment.
    
    \item \textbf{Move around freely in virtual space (within boundaries)}: the XR system should have the capability to assume any realistic or reasonable position within an MR scenario, such as standing in various corners of a room or walking back and forth while engaging in conversation, to facilitate human-like interaction.

    \item \textbf{Display text (on any screen)}: the XR system should have the capability to present standard, two-dimensional text across various types of screens to facilitate the sharing of information.
    
    \item \textbf{Display text (in MR/AR)}: the XR system must have the ability to project text within MR/AR scenarios to facilitate the display of multimedia information.
    
    \item \textbf{Display images (on any screen)}: the XR system should have the capability to present standard image formats across various types of screens to effectively transmit multimedia information.
    
    \item \textbf{Display images (in MR/AR)}: the XR system should have the capability to present standard image formats as seamlessly integrated layers in MR/AR scenarios, facilitating the display of multimedia information.
    
    \item \textbf{Display videos (on any screen)}: the XR system should have the capability to showcase standard video formats across various screen to facilitate the dissemination of multimedia information.
    
    \item \textbf{Display videos (in MR/AR)}: the XR system should have the capability to present standard video formats as smoothly incorporated layers in MR/AR scenarios, facilitating enhanced user experiences.
    
    \item \textbf{Display 3D models (on a screen)}: the XR system should have the capability to present standard 3D models on various screen to effectively display multimedia information.
    
    \item \textbf{Display 3D models (in MR, AR)}: the XR system should have the capability to present standard 3D models as smoothly incorporated layers in MR/AR environments, enabling users to adjust their size, to effectively showcase and customize multimedia information.
\end{itemize}
\subsubsection{NFR}
\label{subsec:env_NFR}
\begin{itemize}
    %POSTE 2
    \item \textcolor{red}{\textbf{Meeting-booking system integration}:}
    \begin{itemize}
        \item Description: meeting-booking system integration;
        \item Rationale: need it to be able to verify the meeting approval.
    \end{itemize}
    \item \textcolor{red}{\textbf{Access control system integration}:}
    \begin{itemize}
        \item Description: access control system integration;
        \item Rationale: need it to be able to enable access.
    \end{itemize} 
\end{itemize}


\subsection{INTERACTION REQUIREMENTS}
\label{subsec:interaction_req}
\subsubsection{FR}
\label{subsec:interaction_FR}
\begin{itemize}
    \item \textbf{Allow user to create an account}: the XR system should support basic account management functionalities to enable user identification and progress saving.
    
    \item \textbf{Allow user to log in to an account}: the XR system should support basic account management functionalities for user identification and progress saving purposes.
    
    \item \textbf{Allow user to create, load and save a procedure}: the XR system must support basic account management functionality to allow creating, uploading and saving the progress of a procedure (e.g.: information activity).
    
    \item \textbf{Greet user}: the XR system should greet the user using the most appropriate manner for the identified user class;
    
    \item \textbf{Allow user to select (main) mode of interaction}: the XR system should offer users a choice of text/touch, voice, and/or gesture interaction methods to tailor interaction to individual preferences.
    
    \item \textbf{Allow user to interact via text/touch}: the XR system must capture and analyze text and touch interactions performed by the user to tailor the interaction to individual users.
    
    \item \textbf{Allow user to interact via voice}: the XR system must be able to recognize and process voice commands initiated by the user to customize interaction according to individual preferences.
    
    \item \textbf{Allow user to interact via gestures}: the XR system must be able to recognize and interpret user-initiated gesture interactions to tailor the interaction experience to individual users.
    
    \item \textbf{Offer multiple choice quizzes}: the XR system should have the capability to present questions in the form of quizzes with multiple options for answering, aiming to engage users while ensuring responsiveness.
    
    \item \textbf{Evaluate user quiz input}: the XR system should be capable of assessing the accuracy of user-provided answers, categorizing them as correct, partially correct, or incorrect, and providing concise explanations, aiming to offer information and identify additional user needs.
    
    \item \textbf{Propose interaction}: the system must offer users the ability to advance, pause, or exit the quiz session, thus tailoring the interaction to the specific needs of the user.
    
    \item \textbf{Show user how to get to a specific location}: the XR system should be able to display a map and provide guidance to the user on navigating from point A to point B to assist users in navigating the XR environment.
    
    \item \textbf{Offer help / background / safety info}: the XR system must be able to offer the user additional assistance and guidance on training at any stage of the experience, with the goal of helping the user.
    \item \textbf{Request operator intervention}: the XR system must allow users to call the security advisor/trainer at any time during the experience, at the user's request, with the goal of facilitating access to outside assistance.
    
    \item \textbf{Allow user to create and log in to content management system (CMS) account}: the backend of the XR system must support basic account management to enable trainers to manage accounts.
        
    \item \textbf{Allow users to create, edit and save training(s)}: the backend of the XR system must provide basic authoring capabilities, enabling users to create, edit, and save training(s).
    
    \item \textbf{Allow import of all standard media types (included 3D models)}: the XR system backend should provide fundamental authoring capabilities, enabling trainers to manage accounts and populate them with various forms of information and multimedia content.
    
    \item \textbf{Provide dashboard}: the backend of the XR system should provide fundamental authoring capabilities, which include database management, role administration, data and resource management, quiz creation, and object interaction templates, allowing trainers to manage accounts and populate them with information and multimedia content.
    
    \item \textbf{Language interaction}: the XR system will possess the capability to use a customized language (e.g., tailored to the user's age) to adapt interactions accordingly.
    
    \item \textbf{Multi-language communication}: users will have the possibility to choose their preferred language for communications, enabling interaction adaptation based on the user's language preference.
    
    \item \textcolor{red}{\textbf{Question Answering}}
    \begin{itemize}
        \item Description: the system will be able to provide information about Financial product like: Bank account or pre-paid card. Its ability to answer has origin in the services documents;
        \item Rationale: provide informative services.
    \end{itemize}
    
    \item \textbf{Engaged and effective communication}:the XR system is designed to interact with the user fluidly and dynamically, incorporating human-like tones, expressions, and conversational skills to enhance the intelligence of artificial intelligence dialogue (e.g., maintaining eye contact, showing interest in the conversation, and adjusting facial expressions according to the topic), with the goal of achieving human-like interaction.
    

    \item \textbf{Ticket Request}: at the end of the question and answer session (information activity), the XR system asks the user to request the release of a ticket, in line with the use case service.
    
    \item \textbf{Request understanding}: the XR system should be able to encompass various requests, such as accessing the building, locating specific areas within the building, accessing security information, or receiving directions to particular locations within the building, all aimed at meeting user needs.

    \item \textbf{Interaction}: the XR system is expected to have an interface for interacting that will include both voice and touch/video modes, enabling more human-like conversation through natural language understanding and recognition of user intent, as well as the ability to access services. The system will respond verbally and simultaneously display information on the screen to ensure appropriate and involving communication, thereby improving user engagement and satisfaction.

    \item \textbf{Guide Proposal}: the physical XR system should offer visitors the option of being accompanied to provide a guide service, thus facilitating navigation to the desired destination.

    \item \textbf{On request safety info}: the XR system must provide relevant information and/or company security regulations, deemed useful or essential for building access, upon request.
\end{itemize}
    
\subsubsection{NFR}
\label{subsec:interaction_NFR}
\begin{itemize}
    \item \textbf{Promotional messages}: the XR system will be capable of suggesting, following user interaction with a service/product, and if applicable, offering a promotion on the service/product discussed, aimed at providing commercial incentives.

    \item \textbf{Sentiment analysis}: the XR system should be able to perform sentiment analysis on detecting users' negative conversations to better understand their satisfaction.
    
    \item \textbf{Look and feel}: the XR system will have its own on-screen representation to enhance user engagement, will be designed to create a pleasant experience, and will express itself through voice messages synchronized with facial expressions and body movements, with the goal of transmitting attention and helpfulness to provide service, all to facilitate effective communication and user engagement.
\end{itemize}


\subsection{OPERABILITY REQUIREMENTS}
\label{subsec:operability_req}
\subsubsection{FR}
\label{subsec:operability_FR}
\begin{itemize}
    \item \textbf{User detection}: the XR system must autonomously detect approaching visitors, defined as individuals who move toward and stop in front of it, excluding passing visitors, to initiate interaction and ensure secure building access.
    
    \item \textbf{Transcribe user requests (voice)}: the XR system should possess the capability to convert user's spoken commands into written, utilizing functionalities such as speech-to-text (STT), to facilitate user interaction and data processing.
    
    \item \textbf{Environment resilience}: the XR system is required to ignore background voices and noise, ensuring they are not mistakenly interpreted as verbal input.

    \item \textbf{Map presentation}: the XR system must be able to display an on-screen presentation of the environment map.
    
    \item \textbf{Movement in environment}: the XR system should support the user in orientation within the environment by displaying an internal map on the screen to help him or her find their way around.
    
    \item \textbf{Information and filling forms}: the XR system should provide information and assistance to users in filling out forms, including the ability to receive customer data (e.g.: via an integrated digital keyboard).
    
    
    \item \textbf{Provide needed information}: the XR system will have the capability to provide needed information through the most suitable means of interaction, including natural language, displayed text, video, and gesture interface, ensuring information dissemination in the most effective manner.
    
    \item \textbf{Gesture}: the XR system must interact with gestures to facilitate human-like interaction.
    
    \item \textbf{Monitor environment}: the XR system should be able to provide monitoring of environmental parameters such as humidity, temperature, brightness, noise, etc. 
    
    \item \textcolor{red}{\textbf{Consultant Availability}}
    \begin{itemize}
        \item Description: at the end of a Q\&A about bank accounting, the system must be able to show the availability calendar of the financial advisor. The user must be able to book an appointment ;
        \item Rationale: booking an appointment in the use case.
    \end{itemize}
    
    \item \textcolor{red}{\textbf{More guests at once}}
    \begin{itemize}
        \item Description: following the presentation of a QR code, the system retrieves the meeting information, including the possible presence of more guests. The system should check for multiple guests to minimize approval calls to the host; 
        \item Rationale: get approval from host and simplify access procedure.
    \end{itemize}
    \item \textbf{User verification}: the XR system should incorporate a user verification process that involves sending an e-mail to the guest containing a link as a second authentication factor along with the QR code, with the goal of obtaining authorization by confirming that the user receiving the reservation-QR is indeed the same one who wishes to access the building.
    
    \item \textcolor{red}{\textbf{Instructions for reaching a location}}
    \begin{itemize}
        \item Description: the system will be able to provide information regarding the location (e.g.: building, room and how to reach it) of the host with whom the visitor has an appointment;
        \item Rationale: simplify reachability of hosts and meeting rooms.
    \end{itemize}
    \item \textcolor{red}{\textbf{Host location}}
    \begin{itemize}
        \item Description: the system has a mapping of the building employees and their location;
        \item Rationale: simplify reachability of hosts and meeting rooms.
    \end{itemize}
    \item \textcolor{red}{\textbf{Meeting room location}}
    \begin{itemize}
        \item Description: the system has a mapping of the meeting rooms and their location; 
        \item Rationale: simplify reachability of hosts and meeting rooms.
    \end{itemize}
    
    \item \textbf{Guiding}: The XR system should be able to accompany visitors within the environment, able to retrieve the target destination, orient itself, select the optimal route, and alert visitors if they deviate from the route, prioritizing safety by avoiding obstacles.
    
\end{itemize}
\subsubsection{NFR}
\label{subsec:operability_NFR}
\begin{itemize}
    \item \textcolor{red}{\textbf{Release ticket number}}
    \begin{itemize}
        \item Description: the system will be able to release the ticket number according to the type of service. When issuing the ticket, the system must be able, on the basis of the interactions it has had with the user, to understand the service for which it should print the ticket;
        \item Rationale: provide ticket number.
    \end{itemize}
    \item \textcolor{red}{\textbf{Paper forms distribution}}
    \begin{itemize}
        \item Description: the system will be able to provide the correct form to the user when needed;
        \item Rationale: provide documentation.
    \end{itemize}
   
    \item \textcolor{red}{\textbf{Package measurement}}
    \begin{itemize}
        \item Description: the agent must be able to scan package’s weight and dimensions;
        \item Rationale: for pre-acceptance of parcel shipping.
    \end{itemize}
    
    \item \textcolor{red}{\textbf{Print document}}
    \begin{itemize}
        \item Description: the system must be able to print documents (e.g., ticket, waybill, ISEE forms);
        \item Rationale: give the users the necessary document to assess to services.
    \end{itemize}
\end{itemize}


\subsection{PERCEPTION REQUIREMENTS}
\label{subsec:perception_req}
\subsubsection{FR}
\label{subsec:perception_FR}
\begin{itemize}
    %POSTE2
    \item \textbf{QR code scan}: the XR system should possess the capability to scan a QR code and verify the associated information. This functionality aims to reduce dependence on physical badges and speed up user recognition.

    \item \textbf{Detect user}: the system must possess the capability to identify the presence of a user to facilitate the beginning of interaction.
    
    \item \textbf{Detect user's indecision}: the XR system should be able to sense the user's indecision during use and should possess a mechanism to suggest an assistance function to the user so as to help him or her.
    
    \item \textbf{Detect help and understand request}: the XR system must recognize when a visitor explicitly asks for assistance in understanding his or her request, whether it is expressed in  language, or through gestural interfaces, to improve user understanding.

    \item \textbf{Recognize user speaking}: the XR system will have the capability to identify the user who is speaking to it, particularly in scenarios where multiple users are present, to initiate interaction with the appropriate user.

    \item \textbf{User classification}: the XR system should be able to classify a visitor based on key characteristics extracted from the detected approaching visitor (e.g., age), facilitating the tailoring of social interaction to the specific user.
    
    \item \textbf{Understand context/intent}: the XR system must possess the ability to recognize differences in user responses and correlate the responses with previously collected data from the user's session to improve engagement, responsiveness, and data processing.
    
    \item \textbf{Detect object}: the XR system must identify whether the user is holding an object (such as a package), and the interaction is initiated only at the user's request, to offer support when requested.
    
    \item \textbf{Handle physical objects presented by user}: the XR system should have the ability to interact with objects presented by the user to enhance user interaction and engagement.
    
    \item \textbf{Capturing end-user feedback}: the XR system should be able to perceive user acceptance and user experience feedback to understand user satisfaction.
\end{itemize}
\subsubsection{NFR}
\label{subsec:perception_NFR}
\begin{itemize}
    \item \textbf{Ease of use}: the user should perceive the XR system as easy to use and comprehend, aiming to enhance user satisfaction and minimize errors.
    
    \item \textbf{Perceived usefulness}: the user must perceive the XR system as useful, to increase the likelihood of its use.
    
    \item \textbf{Perceived reliability}: the user should have the perception of reliability of the XR system, to increase the probability of its use.
\end{itemize}


\subsection{PRIVACY REQUIREMENTS}
\label{subsec:privacy_req}
\subsubsection{FR}
\label{subsec:privacy_FR}
\begin{itemize}
    \item 
\end{itemize}
\subsubsection{NFR}
\label{subsec:privacy_NFR}
\begin{itemize}
    %POSTE 1
    \item \textbf{Privacy for requests}: the XR system will ensure privacy for requests, aligning with both legal mandates and company policies.
    
    \item \textbf{Privacy for responses}: the XR system will ensure privacy for responses, aligning with both legal mandates and company policies.
    
    \item \textbf{Data storage}: data used for body tracking, facial landmarks, or any other information classified as ``personal data'' must be anonymized and not retained, in line with legal and corporate regulations.
    
    \item \textbf{Data processing consent}: the data processed by the XR system must not exceed a real need and must be such that it does not require the user to give explicit consent to data processing, in line with legal and corporate regulations.
    
    \item \textbf{Biometric data processing}: in cases where the XR system requires biometric data, either directly or indirectly linked to identification data, explicit consent for data processing is necessary, even if the biometric data is not stored within the system, in line with legal and corporate regulations.
    
    \item \textbf{Trust}: the user must be assured that interactions with the XR system are safe with regard to the processing of personal data or, at the very least, the perceived risk associated with inappropriate data handling must be minimal in order to increase the likelihood of its use.
    
    \item \textbf{Privacy}: Ensure users' confidentiality of information exchanged during interactions with the XR system, thus preventing unauthorized access to input/output data, in accordance with legal and corporate standards.
    
\end{itemize}


\subsection{REGULATIONS REQUIREMENTS}
\label{subsec:reg_req}
\subsubsection{FR}
\label{subsec:reg_FR}
\begin{itemize}
    \item 
\end{itemize}
\subsubsection{NFR}
\label{subsec:reg_NFR}
\begin{itemize}
    %POSTE 1
    \item \textbf{Sanitary regulations}: use and operation of the XR system must fully comply with health regulations to prevent the spread of viruses and bacteria, in accordance with company policies.
    
    \item \textbf{Accessibility}: the 3D Avatar XR system must adhere to digital accessibility standards (e.g., Low 4 09/01/2004) to meet legal and company requirements.

    \item \textbf{Corporate regulation}: the XR system must adhere to corporate security and safety regulations to meet legal and company requirements.
    
    \item \textbf{Noninvasive job}: the XR system must not disrupt or intrude upon the tasks performed by reception employees, in accordance with company requirements.
\end{itemize}


\subsection{SAFETY REQUIREMENTS}
\label{subsec:safety_req}
\subsubsection{FR}
\label{subsec:safety_FR}
\begin{itemize}
    \item \textbf{Do (mandatory) safety brief}: the XR system must provide instructions to the user on safely operating the system, including handling head-mounted displays (HMDs), with the aim of guiding the user safely through the experience.
        
    \item \textbf{Mandatory safety brief}: the XR system must provide visitors with essential information on security and/or business regulations required for access to the building before granting them entry, ensuring compliance with organizational guidelines.
    
\end{itemize}
\subsubsection{NFR}
\label{subsec:safety_NFR}
\begin{itemize}
    \item \textbf{Signalling}: the XR system must have the capability to alert human operators to abnormal environmental parameters, aiming to enhance environmental quality.
    
    \item \textbf{Physical safety}: the XR system must possess features to ensure: i) sufficient visibility to prevent tripping hazards by the user; ii) measures to prevent accidental collisions with people; and iii) an anti-tilt design, in accordance with legal and corporate regulations.
    
    \item \textbf{Corporate regulation}: the XR system must not impede the regular movements of employees and visitors, in accordance with legal and company requirements.
    
    \item \textbf{Acoustic signal}: the XR system must be equipped with an audible signal or similar measure that activates during movement to signal its presence to people;
    
    \item \textbf{Redundance of sensors}: the XR system should be equipped with redundance sensors to minimize the risk of personal injury.
    
    \item \textbf{Mobile Module deactivation}: it should be feasible to remotely deactivate the XR system in case of potentially harmful behavior, aligning with company policy requirements and aiming to mitigate the risk of personal injury.
    
    \item \textbf{Mobile Module motion}: in the case of physical system XR, security personnel must be present along the system routes in accordance with company policy requirements and to minimize the risk of personal injury.
    
\end{itemize}
